GCNIDS: Graph Convolutional Network-Based Intrusion Detection System for CAN Bus

The Controller Area Network (CAN) bus serves as a standard protocol for facilitating communication among various electronic control units (ECUs) within contemporary vehicles. However, it has been demonstrated that the CAN bus is susceptible to remote attacks, which pose risks to the vehicle's safety and functionality. To tackle this concern, researchers have introduced intrusion detection systems (IDSs) to identify and thwart such attacks. In this paper, we present an innovative approach to intruder detection within the CAN bus, leveraging Graph Convolutional Network (GCN) techniques as introduced by Zhang, Tong, Xu, and Maciejewski in 2019. By harnessing the capabilities of deep learning, we aim to enhance attack detection accuracy while minimizing the requirement for manual feature engineering. Our experimental findings substantiate that the proposed GCN-based method surpasses existing IDSs in terms of accuracy, precision, and recall. Additionally, our approach demonstrates efficacy in detecting mixed attacks, which are more challenging to identify than single attacks. Furthermore, it reduces the necessity for extensive feature engineering and is particularly well-suited for real-time detection systems. To the best of our knowledge, this represents the pioneering application of GCN to CAN data for intrusion detection. Our proposed approach holds significant potential in fortifying the security and safety of modern vehicles, safeguarding against attacks and preventing them from undermining vehicle functionality.

==> Section/name.tex <==
% A real-time behavior detection system has been presented in this article \cite{zhang2018real} using millimeter-wave radar. mmWave Radar was used here for sensing the micro-Doppler information of targets. Later, they implemented a convolution neural network (CNN) in the detection
% and classification of the human motion behaviors using this information.


% A milliMap has been proposed \cite{lu2020see} which is a single-chip millimeter wave (mmWave) radar-based
% indoor mapping system targetted towards low-visibility environments to assist in emergency response. There is a unique feature of milliMap that it does not leverage at a low cost but can reconstruct a dense grid map with accuracy comparable to lidar. It also provides semantic annotations of objects on
% the map.

% A robot mounted millimeter wave (mmWave)
% radar system named mBeats has been propoesd \cite{zhao2020heart}. mBeats provides periodic heart rate measurements
% under different user poses. It does not interfere in a users
% daily activities. Features from mBeats feed into a deep neural network
% predictor which can estimate heart rate. 

% Zhao et al. proposed a human
% tracking and identification system (mID) based on millimeter-wave radar which has a high tracking accuracy, without being
% visually compromising \cite{zhao2019mid}. It is capable of tracking
% and identifying multiple people simultaneously unlike competing techniques based on
% WiFi Channel State Information. Using a deep neural network, they recognize the users individually.


% Jin et al. proposed a novel patient behavior detection system
% using mmWave radar and a deep convolution neural network
% (CNN) \cite{jin2019multiple}. It can detect the simultaneous recognition of multiple
% patients’ behaviors in real-time. They used a mmWave radar to track multiple patients and detected the
% scattering point cloud of each one. The Doppler
% pattern of the point cloud over a while was collected as
% the behavior signature for each patient.
% Classifying the behavior of each patient, a three-layer CNN model was created.

% A novel approach to
% detect and track human skeletons in real-time using an
% mmWave radar named mm-Pose has been proposed in \cite{sengupta2020mm}. According to them, this is the first method to detect greater than 15 distinct skeletal joints using mmWave radar reflection signals. The proposed
% method has a great number of applications like traffic monitoring
% systems, autonomous vehicles, patient monitoring systems, and defense forces. Here, it detected and tracked the human skeleton for
% effective and preventive decision-making in real-time. The
% use of radar made the system robust to work in adverse weather conditions and adverse lighting.

% \textcolor{red}{APPLICATION:  traffic monitoring
% systems, autonomous vehicles, patient monitoring systems, and defense forces.}

% When used for traffic surveillance, mmWave radar may pick up on the presence of anything with wheels \cite{garcia2018robust}. Rain, fog, or dust won't stop it from doing its job of detection. Not only useful in traffic monitoring systems, mmWave radar is also a helpful tool for autonomous vehicles. It can detect blind spots, hold the brakes in an emergency, and issue warnings for forward accidents \cite{verma2020}. mmWave radar has crucial applications in the medical field. These days, doctors use mmWave radar to figure out a patient's breathing and heart rates \cite{alizadeh2019}. The defense system is also impacted by mmWave radar. The manuscript \cite{richard1976millimeter} explains how mmWave radar can be used in air defense, land defense, and ground-to-air defense systems.





% Chang et al. proposed a new spatial attention fusion (SAF) method for obstacle detection using mmWave radar and vision sensor where the sparsity of radar points was considered \cite{chang2020spatial}. The proposed fusion method was embedded in the feature-extraction stage,
% which leveraged the features of mmWave radar and vision sensor effectively. An attention weight matrix was generated to fuse the vision features based on SAF, which was different from the
% concatenation fusion and element-wise add fusion. Moreover, the proposed SAF can be trained by a deep learning object detection framework. They built a generation model which converts radar points to radar images for neural network training.


% This can be a discussion paper
% Guan et al. demonstrated high-resolution imaging using millimeter Wave radars that functioned even in dense fog \cite{Guan_2020_CVPR}. They took advantage of the fact that mmWave signals have favorable propagation characteristics in low visibility conditions, unlike optical sensors as cameras and LiDARs cannot penetrate through dense fog. Millimeter-wave radars have some cons. It suffers from very low resolution, specularity, and noise artifacts. They introduced a system named HawkEye that leveraged a cGAN architecture to recover high-frequency shapes from raw low-resolution mmWave heat-maps. It addressed challenges specific to the structure and nature of the radar signals involved. They implemented their system on a custom-built mmWave radar platform and demonstrated performance improvement over both standard mmWave radars and other competitive baselines.


% Pose estimation for humans is an important task. Traditional human pose estimation is captured through images or videos, which may suffer from bad light and raise privacy concerns. In this paper \cite{Li2020}, they proposed an accurate human pose estimation system using mmWave radar. Two radar data were used to generate heatmaps. They used CNN to transform two-dimensional heatmaps into a human pose.


% Human activity recognition (HAR) becomes a key research area to understand and identify human behavior. Singh et al. proposed RadHAR, a framework that performs accurate HAR
% using sparse and non-uniform point clouds which utilize
% a sliding time window to accumulate point clouds from a
% mmWave radar \cite{singh2019radhar}. It generated a voxelized representation that
% acts as input to their classifiers. According to them, the proposed system is low-cost.

% Users can control smart homes via speech commands nowadays. However, voice assistants become security risks and privacy disclosures. So malicious actors could confuse genuine users to send smart home speech commands. User verification thus becomes a critical issue for smart home security. Dong et al. proposed a secure method for speaker verification using mmWave radar which could increase the home security \cite{dong2021}. Specifically, they utilized the radar to capture both vocal cord vibration and lip motion for identifying speakers. 

% DATASET
% mmWave radars are being increasingly mounted in commercial vehicles to support new Adaptive Driver Assisted Systems due to their ability to provide high accuracy location, velocity, and angle estimates of objects, largely independent of environmental conditions. Gao et al. have created a large raw radar dataset for various objects under different scenarios \cite{gao2019}. Thereafter, they applied some radar imaging algorithms to validate its capabilities in terms of object recognition.


% Seems non-important to me
% A novel interaction paradigm named ThuMouse aimed to create a gesture-based and touch-free cursor interaction \cite{Li2020lei}. It accurately tracks the motion of fingers in real-time. ThuMouse enables users to move the cursor using frequency-modulated continuous-wave (FMCW) radar. They also showed a proof-of-concept demonstration that functioned as a mouse. This work built a foundation allowing the finger to emulate external input devices such as a joystick and touch-pad.


% This could be one of the future work. but not relevant to this research work
% mmWave radar has been shown as an effective alternate for other sensing techniques due to its functional capability in low visibility, smoke, dusty, and dense fog environment. It is still a great challenge to reconstruct 3D object shapes due to the characteristics of radar data such as sparsity, low resolution, specularity, high noise, and multi-path induced shadow reflections and artifacts. Sun et al. proposed 3D Reconstruction and Imaging via mmWave Radar (3DRIMR) \cite{sun2021}. It was a deep learning-based architecture that could reconstruct the 3D shape of an object. Their architecture consisted of two back-to-back conditional GAN deep neural networks.  The first one generated 2D depth images based on raw radar intensity data whereas the second one generated 3D point clouds depending on the results of the first generator. 

% Relevant to the future work
% Human-vehicle classification plays an important role in advanced driver assistance systems for avoiding the accident. mmWave radar sensor may be used heavily in human-vehicle classification algorithms due to its robustness in severe weather. A new mmWave radar point cloud classification algorithm has been proposed to improve classification accuracy under complex scenes of autonomous driving \cite{zhao2020}. To verify the validity and robustness of the proposed feature vector collecting two datasets for static and moving objects, respectively, and each dataset was taken for pedestrians and vehicles at different distances and angles.


% A mmWave radar algorithm has been presented in \cite{toker2020} to detect moving pedestrians and vehicles. It can differentiate pedestrians from other vehicles on the road.


% very old paper
% Gopalsami et al. discussed the development of a mmWave radar chemical sensor for applications in environmental monitoring and arms-control treaty verification \cite{gopalsami2001}. Here, they investigated the use of fingerprint-type molecular rotational signatures in the mmWave spectrum so that it could sense airborne chemicals. 


% Petkie et al. proposed a radar system for the remote measurement of respiration and heart rates \cite{petkie2009}. A lot of advantages of mmWave radar include a higher sensitivity to small displacements, transmission through the atmosphere and clothing, and the ability to maintain a collimated beam over large distances. 


% The task of verification of an identity based on the human face radar signature has been proposed in \cite{hof2020}. They collected a dataset with the faces of 200 different persons. Then, a neural network-based autoencoder was employed to encode each face.



%%%%%%%%% multi-mpodality%%%%%%%%%%%%%%%%%


% A new radar-camera fusion system has been presented which has taken into consideration the error bounds of the two different coordinate systems from the heterogeneous sensors \cite{zhang2019}. To adapt to the heterogeneous sensors, a new fusion-extended Kalman filter has been utilized. Asynchronous sensors, multi-target tracking, and association have been studied and illustrated in this paper for real-world applications.


% There are lots of deep learning algorithms that have been proposed for image classification and object detection. However, these methods may not be fruitful in many real-world scenarios where the visibility or illumination is poor. mmWave radars can assist cameras under adverse conditions. Shuai et al. proposed milliEye, a lightweight mmWave radar and camera fusion system for robust object detection on the edge platforms \cite{shuai2021millieye}. milliEye has several key advantages over existing sensor fusion
% approaches. According to them, milliEye fused two sensing modalities in a learning-based fashion while it used only a small amount of labeled image/radar data. This made milliEye adapt to highly complex real-world environments. 
 
 
%  \section{Related works}
% A real-time behavior detection system has been presented in this article \cite{zhang2018real} using millimeter-wave radar. mmWave Radar was used here for sensing the micro-Doppler information of targets. Later, they implemented a convolution neural network (CNN) in the detection
% and classification of the human motion behaviors using this information.


% A milliMap has been proposed \cite{lu2020see} which is a single-chip millimeter wave (mmWave) radar-based
% indoor mapping system targetted towards low-visibility environments to assist in emergency response. There is a unique feature of milliMap that it does not leverage at a low cost but can reconstruct a dense grid map with accuracy comparable to lidar. It also provides semantic annotations of objects on
% the map.

% A robot mounted millimeter wave (mmWave) radar system named mBeats has been propoesd \cite{zhao2020heart}. mBeats provides periodic heart rate measurements under different user poses. It does not interfere in a users
% daily activities. Features from mBeats feed into a deep neural network
% predictor which can estimate heart rate. 

% Zhao et al. proposed a human
% tracking and identification system (mID) based on millimeter-wave radar which has a high tracking accuracy, without being
% visually compromising \cite{zhao2019mid}. It is capable of tracking
% and identifying multiple people simultaneously unlike competing techniques based on
% WiFi Channel State Information. Using a deep neural network, they recognize the users individually.


% Jin et al. proposed a novel patient behavior detection system
% using mmWave radar and a deep convolution neural network
% (CNN) \cite{jin2019multiple}. It can detect the simultaneous recognition of multiple
% patients’ behaviors in real-time. They used a mmWave radar to track multiple patients and detected the
% scattering point cloud of each one. The Doppler
% pattern of the point cloud over a while was collected as
% the behavior signature for each patient.
% Classifying the behavior of each patient, a three-layer CNN model was created.

% A novel approach to
% detect and track human skeletons in real-time using an
% mmWave radar named mm-Pose has been proposed in \cite{sengupta2020mm}. According to them, this is the first method to detect greater than $15$ distinct skeletal joints using mmWave radar reflection signals. The proposed method has a great number of applications like traffic monitoring
% systems, autonomous vehicles, patient monitoring systems, and defense forces. Here, it detected and tracked the human skeleton for
% effective and preventive decision-making in real-time. The
% use of radar made the system robust to work in adverse weather conditions and adverse lighting.

% Chang et al. proposed a new spatial attention fusion (SAF) method for obstacle detection using mmWave radar and vision sensor where the sparsity of radar points was considered \cite{chang2020spatial}. The proposed fusion method was embedded in the feature-extraction stage,
% which leveraged the features of mmWave radar and vision sensor effectively. An attention weight matrix was generated to fuse the vision features based on SAF, which was different from the
% concatenation fusion and element-wise add fusion. Moreover, the proposed SAF can be trained by a deep learning object detection framework. They built a generation model which converts radar points to radar images for neural network training.

% Guan et al. demonstrated high-resolution imaging using millimeter Wave radars that functioned even in dense fog \cite{Guan_2020_CVPR}. They took advantage of the fact that mmWave signals have favorable propagation characteristics in low visibility conditions, unlike optical sensors as cameras and LiDARs cannot penetrate through dense fog. Millimeter-wave radars have some cons. It suffers from very low resolution, specularity, and noise artifacts. They introduced a system named HawkEye that leveraged a cGAN architecture to recover high-frequency shapes from raw low-resolution mmWave heat-maps. It addressed challenges specific to the structure and nature of the radar signals involved. They implemented their system on a custom-built mmWave radar platform and demonstrated performance improvement over both standard mmWave radars and other competitive baselines.


% Pose estimation for humans is an important task. Traditional human pose estimation is captured through images or videos, which may suffer from bad light and raise privacy concerns. In this paper \cite{Li2020}, they proposed an accurate human pose estimation system using mmWave radar. Two radar data were used to generate heatmaps. They used CNN to transform two-dimensional heatmaps into a human pose.


% Human activity recognition (HAR) becomes a key research area to understand and identify human behavior. Singh et al. proposed RadHAR, a framework that performs accurate HAR
% using sparse and non-uniform point clouds which utilize
% a sliding time window to accumulate point clouds from a
% mmWave radar \cite{singh2019radhar}. It generated a voxelized representation that
% acts as input to their classifiers. According to them, the proposed system is low-cost.

% Users can control smart homes via speech commands nowadays. However, voice assistants become security risks and privacy disclosures. So malicious actors could confuse genuine users to send smart home speech commands. User verification thus becomes a critical issue for smart home security. Dong et al. proposed a secure method for speaker verification using mmWave radar which could increase the home security \cite{dong2021}. Specifically, they utilized the radar to capture both vocal cord vibration and lip motion for identifying speakers. 

% mmWave radars are being increasingly mounted in commercial vehicles to support new Adaptive Driver Assisted Systems due to their ability to provide high accuracy location, velocity, and angle estimates of objects, largely independent of environmental conditions. Gao et al. have created a large raw radar dataset for various objects under different scenarios \cite{gao2019}. Thereafter, they applied some radar imaging algorithms to validate its capabilities in terms of object recognition.


% A novel interaction paradigm named ThuMouse aimed to create a gesture-based and touch-free cursor interaction \cite{Li2020lei}. It accurately tracks the motion of fingers in real-time. ThuMouse enables users to move the cursor using frequency-modulated continuous-wave (FMCW) radar. They also showed a proof-of-concept demonstration that functioned as a mouse. This work built a foundation allowing the finger to emulate external input devices such as a joystick and touch-pad.


% mmWave radar has been shown as an effective alternate for other sensing techniques due to its functional capability in low visibility, smoke, dusty, and dense fog environment. It is still a great challenge to reconstruct 3D object shapes due to the characteristics of radar data such as sparsity, low resolution, specularity, high noise, and multi-path induced shadow reflections and artifacts. Sun et al. proposed 3D Reconstruction and Imaging via mmWave Radar (3DRIMR) \cite{sun2021}. It was a deep learning-based architecture that could reconstruct the 3D shape of an object. Their architecture consisted of two back-to-back conditional GAN deep neural networks.  The first one generated 2D depth images based on raw radar intensity data whereas the second one generated 3D point clouds depending on the results of the first generator. 

% Human-vehicle classification plays an important role in advanced driver assistance systems for avoiding the accident. mmWave radar sensor may be used heavily in human-vehicle classification algorithms due to its robustness in severe weather. A new mmWave radar point cloud classification algorithm has been proposed to improve classification accuracy under complex scenes of autonomous driving \cite{zhao2020}. To verify the validity and robustness of the proposed feature vector collecting two datasets for static and moving objects, respectively, and each dataset was taken for pedestrians and vehicles at different distances and angles.


% A mmWave radar algorithm has been presented in \cite{toker2020} to detect moving pedestrians and vehicles. It can differentiate pedestrians from other vehicles on the road.


% Gopalsami et al. discussed the development of a mmWave radar chemical sensor for applications in environmental monitoring and arms-control treaty verification \cite{gopalsami2001}. Here, they investigated the use of fingerprint-type molecular rotational signatures in the mmWave spectrum so that it could sense airborne chemicals. 


% Petkie et al. proposed a radar system for the remote measurement of respiration and heart rates \cite{petkie2009}. A lot of advantages of mmWave radar include a higher sensitivity to small displacements, transmission through the atmosphere and clothing, and the ability to maintain a collimated beam over large distances. 


% The task of verification of an identity based on the human face radar signature has been proposed in \cite{hof2020}. They collected a dataset with the faces of 200 different persons. Then, a neural network-based autoencoder was employed to encode each face.



% %%%%%%%%% multi-mpodality%%%%%%%%%%%%%%%%%


% A new radar-camera fusion system has been presented which has taken into consideration the error bounds of the two different coordinate systems from the heterogeneous sensors \cite{zhang2019}. To adapt to the heterogeneous sensors, a new fusion-extended Kalman filter has been utilized. Asynchronous sensors, multi-target tracking, and association have been studied and illustrated in this paper for real-world applications.


% There are lots of deep learning algorithms that have been proposed for image classification and object detection. However, these methods may not be fruitful in many real-world scenarios where the visibility or illumination is poor. mmWave radars can assist cameras under adverse conditions. Shuai et al. proposed milliEye, a lightweight mmWave radar and camera fusion system for robust object detection on the edge platforms \cite{shuai2021millieye}. milliEye has several key advantages over existing sensor fusion
% approaches. According to them, milliEye fused two sensing modalities in a learning-based fashion while it used only a small amount of labeled image/radar data. This made milliEye adapt to highly complex real-world environments. 

==> Section/unnecessary.tex <==
\section{Problem Statement}
In this research work, we specifically address the shortcomings of conventional RGB image-based object detection approaches in the presence of occlusion due to low visibility and ambient variability. Also, when it comes to dealing with sensitive personal information, image-based models may give rise to serious privacy concerns in this detection process. We propose the use of mmWave radar in such scenarios as it not only provides viable solutions to those aforementioned issues but also offers an inherent ability to detect millimeter-scale object movements.
We have specified the following research questions to be investigated:
\begin{enumerate}[i.]
    \item How does an object detection mode perform when the objects of interest are placed in an occluded environment or visibility is compromised?
    \item What is the optimum vertical distance between the mmWave radar and the object to secure an accurate detection?
    \item How transferable the features are when we train the model with data from one ambience and try to conduct the inference in a different ambience?
\end{enumerate}
In an endeavor to answer those questions, we have compiled a comprehensive dataset collected using our customized robotic agent equipped with an mmWave radar, considering two important aspects: ambience and height, for five different classes. We also present empirical analysis on the transferability of features in a cross-ambience scenario.

%%%%% static

FCL = [0.952, 0.930, 0.912, 0.300, 0.296, 0.464, 0.328, 0.621, 0.518, 0.991, 0.891, 0.856, 0.157, 0.361, 0.128, 0.411, 0.177, 0.237]
CNN = [0.998, 0.981, 0.952, 0.472, 0.443, 0.484, 0.541, 0.550, 0.448, 0.995, 0.991, 0.863, 0.191, 0.209, 0.286, 0.356, 0.255, 0.317]
UDA = [-, -, -, 0.422, 0.556, 0.509, 0.226, 0.533, 0.511, -, -, -, 0.235, 0.677, 0.273, 0.718, 0.271, 0.251]
SSDA_10 = [-, -, -, 0.660, 0.625, 0.636, 0.611, 0.681, 0.724, -, -, -, 0.536, 0.784, 0.471, 0.798, 0.469, 0.618]
SSDA_20 = [-, -, -, 0.676, 0.822, 0.706, 0.708, 0.851, 0.773, -, -, -, 0.552, 0.819, 0.574, 0.828, 0.688, 0.828]




%%%%% dynamic


fcl = [0.884, 0.901, 0.931, 0.347, 0.488, 0.662, 0.433, 0.653, 0.355, 0.628, 0.771, 0.723, 0.754, 0.431, 0.416, 0.582, 0.311, 0.587, 0.350, 0.547]

cnn = [0.998, 0.985, 0.983, 0.351, 0.455, 0.691, 0.456, 0.668, 0.382, 0.663, 0.841, 0.854, 0.873, 0.440, 0.327, 0.524, 0.328, 0.589, 0.420, 0.577]

uda = [-, -, -, 0.365, 0.589, 0.697, 0.472, 0.792, 0.508, -, -, -, -, 0.450, 0.389, 0.618, 0.404, 0.593, 0.434, -]

ssda_10 = [-, -, -, 0.689, 0.651, 0.861, 0.687, 0.831, 0.565, -, -, -, -, 0.511, 0.445, 0.688, 0.484, 0.661, 0.536, -]

ssda_20 = [-, -, -, 0.716, 0.771, 0.898, 0.786, 0.864, 0.725, -, -, -, -, 0.559, 0.506, 0.698, 0.528, 0.714, 0.602, -]

